Qubit Mapping Based on Subgraph Isomorphism and Filtered Depth-Limited Search

Mapping logical quantum circuits to Noisy Intermediate-Scale Quantum (NISQ) devices is a challenging problem which has attracted rapidly increasing interests from both quantum and classical computing communities. This paper proposes an efficient method by (i) selecting an initial mapping that takes into consideration the similarity between the architecture graph of the given NISQ device and a graph induced by the input logical circuit; and (ii) searching, in a filtered and depth-limited way, a most useful SWAP combination that makes executable as many as possible two-qubit gates in the logical circuit. The proposed circuit transformation algorithm can significantly decrease the number of auxiliary two-qubit gates required to be added to the logical circuit, especially when it has a large number of two-qubit gates. For an extensive benchmark set of 131 circuits and IBM's current premium Q system, viz., IBM Q Tokyo, our algorithm needs, in average, 0.4346 extra two-qubit gates per input two-qubit gate, while the corresponding figures for three state-of-the-art algorithms are 0.6047, 0.8154, and 1.0067 respectively.

==> filter_table.tex <==
\vspace*{-5mm}
\begin{table*}[htbp]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
    \multirow{2}*{$Q$-filter}&\multicolumn{2}{c|}{small}& \multicolumn{2}{c|}{medium}& \multicolumn{2}{c|}{large} & \multicolumn{2}{c}{all}\\
\cline{2-9}
& index & time (s) &index & time (s) &index & time (s) &index & time (s)\\ \hline
$Q_0$  & 1.2694 & 7 & 1.3817 & 112 &1.4741& 28517&1.4702 & 28636 \\
$Q_0$ \& $Q_1$ & 1.2545  & 6 & 1.3718 & 58 & 1.4376 &6928& 1.4346& 6992\\
$Q_0$ \& weak $Q_1$ & 1.2422 & 14 & 1.2946 & 139 & 1.3921 & 35280 &1.3886 & 35433 \\
weak $Q_1$ &1.2162 & 22 &1.2752 & 184 &1.3553& 46553 & 1.3523 & 46759 \\
none  & 1.2138 & 379 &1.2742 &5142 &-&- &-&- \\
%\hline
\end{tabular}
\caption{Summary of the performance of our algorithm with different filters, where the `none' row uses no filters, the `$Q_0$' row (the `weak $Q_1$' row, resp.) uses $Q_0$-filter (`weak $Q_1$' filter, resp.) for all  {\swap}s, and the `$Q_0$ \& $Q_1$' row (the `$Q_0$ \& weak $Q_1$' row, resp.) uses $Q_0$-filter for the first {\swap} and $Q_1$ (weak $Q_1$-filter, resp.) for the rest {\swap}s. } \label{tab:filters}
\end{table*}
